Magnetic Manifold Hamiltonian Monte Carlo

Markov chain Monte Carlo (MCMC) algorithms offer various strategies for sampling; the Hamiltonian Monte Carlo (HMC) family of samplers are MCMC algorithms which often exhibit improved mixing properties. The recently introduced magnetic HMC, a generalization of HMC motivated by the physics of particles influenced by magnetic field forces, has been demonstrated to improve the performance of HMC. In many applications, one wishes to sample from a distribution restricted to a constrained set, often manifested as an embedded manifold (for example, the surface of a sphere). We introduce magnetic manifold HMC, an HMC algorithm on embedded manifolds motivated by the physics of particles constrained to a manifold and moving under magnetic field forces. We discuss the theoretical properties of magnetic Hamiltonian dynamics on manifolds, and introduce a reversible and symplectic integrator for the HMC updates. We demonstrate that magnetic manifold HMC produces favorable sampling behaviors relative to the canonical variant of manifold-constrained HMC.

==> algorithms/euclidean-integrator.tex <==
\begin{algorithm}[t!]
\caption{The procedure for integrating Euclidean magnetic Hamiltonian trajectories. This method is from \cite{pmlr-v70-tripuraneni17a} and \cite{leimkuhler_reich_2005}.}
\label{alg:euclidean-integrator}
\begin{algorithmic}[1]
\State \textbf{Parameters}: Hamiltonian $H(q, p) = U(q) + \frac{1}{2} p^\top p$. 
\State \textbf{Input}: Initial position and momentum variables $q_0\in\R^m$ and $p_0\in\R^m$. Integration step-size $\epsilon$ and number of integration steps $N\in\mathbb{N}$. Skew-symmetric matrix $\mathrm{L}\in\text{Skew}(m)$.
\For{$n = 0,\ldots, N-1$}
    \State Compute $(q_{n+1}, p_{n+1})$ using \cref{alg:euclidean-single-step} with input $(q_{n}, p_{n})$, step-size $\epsilon$, and skew-symmetric matrix $\mathrm{L}$.
\EndFor
\State \textbf{Return}: $(q_N, p_N)$.
\end{algorithmic}
\end{algorithm}

==> theory/cor-detailed-balance-mmhmc.tex <==
\ifappendix
\begin{corollary*}
\else
\begin{corollary}\label{cor:detailed-balance-mmhmc}
\fi
Under the assumptions of \cref{thm:detailed-balance}, a Markov chain whose transition operator is given by \cref{alg:mmhmc} with inputs $(q, p)\in\mathrm{T}^*M$, number of integration steps $N$, and skew-symmetric matrix $\mathrm{L}$ is stationary for the distribution $\pi(q,p) \propto e^{-H(q, p)}$.
\ifappendix
\end{corollary*}
\else
\end{corollary}
\fi
